CFT-Forensics: High-Performance Byzantine Accountability for Crash Fault Tolerant Protocols

Crash fault tolerant (CFT) consensus algorithms are commonly used in scenarios where system components are trusted -- e.g., enterprise settings and government infrastructure. However, CFT consensus can be broken by even a single corrupt node. A desirable property in the face of such potential Byzantine faults is \emph{accountability}: if a corrupt node breaks protocol and affects consensus safety, it should be possible to identify the culpable components with cryptographic integrity from the node states. Today, the best-known protocol for providing accountability to CFT protocols is called PeerReview; it essentially records a signed transcript of all messages sent during the CFT protocol. Because PeerReview is agnostic to the underlying CFT protocol, it incurs high communication and storage overhead. We propose CFT-Forensics, an accountability framework for CFT protocols. We show that for a special family of \emph{forensics-compliant} CFT protocols (which includes widely-used CFT protocols like Raft and multi-Paxos), CFT-Forensics gives provable accountability guarantees. Under realistic deployment settings, we show theoretically that CFT-Forensics operates at a fraction of the cost of PeerReview. We subsequently instantiate CFT-Forensics for Raft, and implement Raft-Forensics as an extension to the popular nuRaft library. In extensive experiments, we demonstrate that Raft-Forensics adds low overhead to vanilla Raft. With 256 byte messages, Raft-Forensics achieves a peak throughput 87.8\% of vanilla Raft at 46\% higher latency ($+44$ ms). We finally integrate Raft-Forensics into the open-source central bank digital currency OpenCBDC, and show that in wide-area network experiments, Raft-Forensics achieves 97.8\% of the throughput of Raft, with 14.5\% higher latency ($+326$ ms).

==> apdx/2-liveness.tex <==

\section{\sysnamelive}
\label{sec:liveness}

We provided accountability for Byzantine faults that compromise safety. 
In this section, we ask how to account for liveness attacks.
Although we use a partially synchronous network model that guarantees message arrivals in bounded time, 
the GST is typically unknown.
Consequently, any method that tries to distinguish a late message and a dropped message is unable to achieve 100\% accuracy. 
Therefore, when one node (Alice) claims failure in receiving message from another node (Bob), it is impossible to find out the faulty node between Alice and Bob with irrefutable evidence. 
As a consequence, an attacker can evade exposure if it consistently denies receiving heartbeats from the current leader and starts new elections, paralyzing the system without any honest leader executing log replication. 

In response to such challenges, we aim to \emph{tolerate} Byzantine faults that only compromises liveness in a new design, in addition to accountability for safety attacks in Raft-Forensics and Paxos-Forensics. 
We name the new consensus algorithm \textbf{\sysnamelive} to emphasize its difference from \sysname. 
We consider the typical definition of liveness in partially synchronous SMR protocols, which requires all honest replicas to eventually commit a correct request submitted by a client.  
To guarantee liveness, we assume there exists \textbf{only one} corrupt node that may commit Byzantine faults, and the total number of faulty nodes does not exceed $f$. The protocol design is presented in \sref{sec:liveness-design}. 
Then, we formally prove that \sysnamelive achieves the liveness property. 
Since \sysnamelive makes no changes to log replication compared to \sysname, its performance on average (without leader changes) is the same as in \sref{sec:eval}. 

% \subsection{Model}

%This is motivated by the fact that if there exists a node with Byzantine faults and $f$ \emph{other} honest nodes with crash faults, we can account for safety threats but we cannot tolerate liveness threats that inevitably paralyze the system without enough live honest nodes. 


% We define liveness from the perspective of request processing. 

% % \todo{find other definitions; use names in literature} \xw{Perhaps use the definition from PBFT: https://pmg.csail.mit.edu/papers/osdi99.pdf}
% % \wt{I don't think it's necessary anymore}

% \begin{definition}[Liveness]
%     In a partially-synchronous network, a consensus algorithm is \emph{live} if within bounded time after a client submits a request, the client will receive irrefutable confirmation that request is committed. 
% \label{def:liveness}
% \end{definition}

\subsection{Design}
\label{sec:liveness-design}

% \gfa{It would be nice to add some interpretation of the protocol before describing it, and mention the round robin leadership cycle. That's a nontrivial modification, and an interesting one.}

Table \ref{tab:notations-liveness} shows a list of additional parameters that are used in the system design. 

\begin{table*}[!htb]
    \centering\small
    \begin{tabular}{p{3.6em}p{21em}p{5.6em}}
    \hline
        Symbol & Description & Requirement \\
    \hline
        $\theart$ & Timeout of leader's heartbeats or RPC responses & $ \ge \Delta$ \\
        $\tcand$ & Timeout of candidate during election & $ \ge 2\Delta$ \\
        $\tvoter$ & Timeout of voters during election & $ \ge \tcand + 2\Delta$ \\
        $\tclient$ & Timeout of client's first trial of request submission & $ \ge 4\Delta$ \\
        $\treq$ & Timeout of receiving request commitment certificate & $ \ge 2\Delta$ \\
    \hline
    \end{tabular}
    \caption{Table of Parameters of \sysnamelive. Recall that we assume a partially-synchronous network with max message delay $\Delta$ after GST.}
    \label{tab:notations-liveness}
    \vspace{-0.6cm}
\end{table*}

\subsubsection{Motivation}

In \sysname, the procedure of leader election is almost identical to vanilla Raft, which exposes the protocol to various liveness attacks. 
One of the major flaws is that during leader election, an adversarial node can seize leadership by claiming a highest term among all candidates without any proof or limitation. 
In response, we adopt a \textbf{round-robin} design in place of the vanilla elections, which guarantees the chance of an honest node being elected. 

    Round-Robin leadership rotations are common and secure in BFT protocols such as Hotstuff, but not yet sufficient to guarantee liveness in Raft.
    This is because the leader can be easily changed when a follower claims a timeout without having to show any evidence. 
    Consequently, an adversarial follower can disable every honest leader that is rotated, and seize leadership for itself. 
    To handle this, we design \textbf{prevote}, which tightens the condition of leadership (or candidacy) changes.     

    Round-Robin elections and prevote ensure that if  the current leader is honest, it will be able to serve indefinitely and guard the liveness of the system. 
    However, liveness is still not ensured if the initial leader after GST is adversarial, who can arbitrarily censor client requests without raising suspicion by honest followers. 
    This motivates our final piece---\textbf{client-leader dispute}, which allows honest replicas to impeach the leader in a process with a second trial.     

In summary, \sysnamelive consists of the three pieces mentioned above---round-robin election, prevote and client-leader dispute. 
In Theorem \ref{thm:availability}, we prove that they are sufficient to guarantee liveness against 1 Byzantine node. 

% \sysnamelive can be divided into three major components -- client dispute, prevote and round-robin election. 
% Although they are highly coupled in the system to achieve liveness, we list three examples of liveness attacks that motivate each of them. 
% In detail, Example \ref{eg:censor} shows why clients must be able to issue complaints about the leader. 
% Example \ref{eg:dol} motivates a prevote procedure that prevents a single Byzantine node from using new elections to block an honest leader. 
% Example \ref{eg:vote-mono} motivates a round-robin leader election 
% % that eliminates term wars in a leader election which may grant 
% to prevent adversarial nodes from gaining an indefinite advantage in winning elections. % in Raft and \sysname. 

% \begin{example}[Censorship]
% \label{eg:censor}
%     When a client sends a request to the leader, the leader ignores the request. 
% \end{example}

% \begin{example}[Anarchy]
% \label{eg:dol}
%     Whenever a new leader is elected, an adversarial node claims that the new leader timed out and starts a new election.
% \end{example}

% \begin{example}[Vote Monopoly]
% \label{eg:vote-mono}
%     When a leader election begins, the adversarial node increments its term after an overly-brief timeout period (instead of randomly sampling between 150-300 ms, as honest nodes do).
%     If the adversary receives a quorum, instead of claiming it, the node remains silent, such that each honest node will timeout and revote at a new term. 
%     By protocol, an honest node will not vote for any other node than itself or the adversary. 
%     The election never ends, so the system cannot process client requests. 
% \end{example}

% \paragraph*{Liveness.} 
% Unlike safety attacks, liveness attacks are difficult to account for with irrefutable proofs. 
% For instance, when node $a$ initiates a leader election by claiming that the current leader $\ell$ timed out, it is impossible for $a$ to prove that $\ell$ failed to send a heartbeat in time, or for $\ell$ to prove that $a$ received a recent heartbeat that prevents the timeout. 
% Instead of forcing Byzantine nodes to leave irrefutable traces, we modify Raft to make it \textbf{tolerant} to deadlocking attacks, especially those listed in \sref{sec:properties-liveness}. 


% \subsubsection{Liveness}
% \label{sec:safety-properties-liveness}

% % We list two liveness properties at different levels. 

% % \begin{itemize}
% %     \item \textbf{Weak Availability.} Within a finite period of time (which can be arbitrarily long) after a client submits a request to the servers, it will get a legitimate receipt that request has been processed. 

% %     \item \textbf{Strong Availability.} Within a finite, \emph{upper-bounded} period of time after a client submits a request to the servers, it will get a legitimate receipt that request has been processed. 
% % \end{itemize}


% \begin{example}[Work Piling up]
% \label{eg:work-pile}
%     The leader honestly nodetes every request during its term, but never informs the followers of their commitments. When a new election begins, every honest node has to commit and apply the corresponding log entries, which can be arbitrarily many. This occupies CPU and IO resources and prevents new requests from being processed in time.  
% \end{example}

% % \begin{example}[Vote Oligopoly]
% % \label{eg:vote-olig}
% %     We call an honest node $h$ a dedicated neighbor of adversarial node $a$, if the distance between $a$ and $h$ is less than that between $h$ and any other adversarial node (ties do not exist).
% %     The adversary establishes $\beta \in [2, \alpha]$ nodes, where none of the $\beta$ nodes own more than $n$ dedicated neighbors. 
% %     During a leader election, each adversarial node increments its term after minimal timeout (instead of random sampling between 150 ms and 300 ms for honest nodes). 
% %     As a result, every term of the election always ends with split vote, and the system cannot have a leader to process client requests. 
% % \end{example}
% \begin{example}[Vote Monopoly]
% \label{eg:vote-mono}
%     When a leader election is started, the adversarial node increments its term after minimal timeout (instead of random sampling between 150 ms and 300 ms for honest nodes).
%     Instead of claiming a quorum of votes, the adversarial node remains silent, such that each honest node will timeout and revote at a new term. 
%     However, by the protocol, it will not vote for any other node than itself or the adversary. 
%     As a result, the election never ends up with a node claiming the leadership, and the system cannot have a leader to process client requests. 
% \end{example}

% Examples \ref{eg:dol}, \ref{eg:censor} and \ref{eg:vote-mono} violates weak availability and \eref{eg:work-pile} violates strong availability.
% In practice, it is infeasible to protect strong availability or even detect the culprits that violates it with irrefutable proof. 
% In contrast, to violate weak availability, the adversary must block the system from processing any request. 
% Since blockers are serious threats to Raft and it is also difficult to provide irrefutable proofs for attacks such as \eref{eg:vote-mono}, we aim to redesign Raft such that it is \emph{tolerant} against deadlocking Byzantine faults.  

\subsubsection{Design Details}
\label{sec:live-design}
% \gfa{Are disputes between client and leader the only relevant ones? Why?}
% \gfa{I still don't understand why we only need to account for disputes between a client and a leader. Why can't there be liveness disputes between a follower and a leader?}
% \gf{need to clarify the differences between this approach and byzantine broadcast work by Shi et al}

\paragraph*{Round-Robin Election}
Once the multi-signed prevote is acquired, $v$ broadcasts the multi-signed prevote message to all the other nodes, including the candidate $c_{t+1}$ of the term $t+1$. 
$v$ starts a timer of duration \tvoter that times out after an honest $c_{t+1}$ could sufficiently react to the election. 
$c_{t+1}$ is the only available candidate defined by the protocol that can receive votes and win the election at term $t+1$. 
We choose $c_{t+1} = (t+1)\mod n$, such that the candidacy moves to every node round-robin as the term number increments. 
 
When $c_{t+1}$ enters term $t+1$, it broadcasts a vote request to all the nodes. 
The vote request contains a tuple of log status $(T, J)$, which denotes the term number and height of $c_{t+1}$'s latest log entry, respectively. 
Given this tuple, an honest node $v$ agrees to vote for $c_{t+1}$ if and only if $c_{t+1}$ is as fresh (Definition \ref{def:fresh}) as itself. 
Upon agreement, it signs the request and returns it to the candidate $c_{t+1}$. 
Note that, however, when $c_{t+1}$ enters term $t+1$, it sets its timer with a different duration \tcand, satisfying
%
\[ \tcand \ge 2\Delta,\quad \tvoter \ge \tcand + 2\Delta. \]

Once the candidate $c_{t+1}$ receives $f+1$ votes, it generates a \emph{leader certificate} which is a multi-signature of these voters, and establishes authority by broadcasting the certificate. 
If the candidate fails to do so, nodes time out at term $t+1$, and broadcast prevote messages to start the election of term $t+2$. 

The procedure of the leader election is specified by Algorithm \ref{alg:rf-elect}. 
The following proposition shows than the expected duration of a round-robin election is constant in $n$. 
We present the proof in \S\ref{sec:proof-rr}. 

\begin{proposition}
    Assume that in \sysnamelive, there is no Byzantine faults and at the start of an election, the freshness order of the followers is uniformly distributed. 
    Then, the expected time complexity of a round-robin election is a constant that is irrelevant to the number of nodes $n$. 

    \label{thm:perf-rr}
\end{proposition}



\paragraph*{Prevote} 
% \wt{
After dealing with client-leader disputes, we resolve follower-leader disputes over leader's liveness by prevotes. 
In vanilla Raft and \sysname, a follower can initiate a leader election by simply claiming the leader has timed out, which can be exploited to stop an honest leader from working. 
We use prevotes to prevent adversarial nodes from denying an honest node leadership.  
% }

From the perspective of a follower, when the leader fails to send a heartbeat, respond to RPCs or process a client request in time,  
% Once a follower $v$ detects one of the following cases, 
% a timeout of the heartbeats at term $t$ (or other RPC timeouts such as during a log synchronization request), 
the follower determines that the leader is faulty and broadcasts a signed prevote message for the next term $t+1$. 
A full list of conditions for prevote is listed in \sref{sec:liveness-prevote}. 

% \begin{enumerate}
%     \item The leader fails to send a heartbeat before timeout.
%     \item The leader fails to respond to RPCs before timeout.
%     \item The leader fails to process a client request in time. 
% \end{enumerate}

After broadcasting the message, $v$ hangs and collects prevote messages from other nodes. 
We say that $v$ is \emph{waiting for} term $t+1$. 
When another node $u$ receives such a prevote message, 
% \gfa{who received it? $v$ or someone else?}, 
it will store the prevote but not react if $u$ does not meet the prevote conditions locally. 
On the other hand, if $u$ meets one of the conditions, it will generate another prevote message signed by itself. 
Then combines $v$'s prevote with its own and broadcasts the prevotes. 

Let $w$ be an arbitrary node (can be $u$ or $v$) who obtains $2$ valid prevotes.
$w$ will broadcast them and enter the election of term $t+1$. 
% \gfa{prevotes received at $v$? or total in the whole system?}
% On the other hand, when $v$ collects $2$ prevote messages of the same term in total, it enters the election of term $t+1$. 
Meanwhile, $w$ starts a timer that times out after $\tvoter$. 
We say $w$ is \emph{inside} term $t+1$ before the timeout.
% \gfa{This para is confusing--do the other nodes have to sign $v$'s prevote? Or does it count if they generate their own prevotes and $f+1$ nodes send the prevote to $v$?}

\paragraph*{\modify{Client-Leader Dispute}}
A client submits a request to the system by sending the request to arbitrary nodes. 
A leader processes the request directly, while a follower forwards the request to the current leader.
% \gf{A client submits a request to the system by sending the request to arbitrary nodes. 
% A leader processes the request directly, while a follower forwards the request to the current leader. <--GF: I un-commented this, it's important.}
% Suppose the client is able to monitor the leader admitted by each node, such that when there exists a node admitted by a majority of (at least $f+1$) nodes, {the client} can directly send a request to the leader if it wants a request to be processed. 
% \gfa{Is this an assumption? Under what conditions is it possible? Phrasing is weird}
Suppose the client resubmits a client request periodically if the request is not processed in time. 
This may happen when the leader is faulty, and it causes a timeout. 
Formally, we let the {client's} timeout be \tclient {(i.e., the time it waits after submitting a request before assuming a fault)}.
% We assume \todo{}

Once the {client's} timeout timer expires, the client executes a second try by broadcasting its request to all the nodes, where each follower node forwards the request to the leader. 
Upon seeing a second-trial message, the follower starts a timer {that can be} stopped {only upon receiving both } %by not only 
a replication of the log entry and a \emph{commitment certificate} from the leader. 
% Recall that the certificate contains signatures of at least $f+1$ nodes. 
If a follower does not receive the certificate before timeout, it immediately starts a prevote, announcing that it no longer regards the current leader as legitimate. 
When there exists no more than $f-1$ nodes that still collaborate with the leader, the leader will not be able to commit any request and fall by more complaints from other clients.

% If a follower witnesses a timeout, it sends a signed testimony to the client. 
% With $f+1$ signatures, the client can declare the failure of the second trial caused by the leader with irrefutable proofs.  
% Then, the client broadcasts the multi-signed testimony as an impeachment of the current leader. 
% Such impeachment forces each honest node to initiate a prevote for the next election to overthrow the leader. 

On the other hand, this try-again mechanism is safe when the client is adversarial and the leader is honest. 
Each honest follower will receive the commitment certificate in time from the honest leader, so the honest leadership authority will remain. 
% The client will not be able to obtain the testimonies required to overthrow the leader, since the leader will process each request submitted by the client honestly and no follower complains about it. 

%  honest node will immediately initiate a prevote after receipt. 
%\xw{What will happen if the client did not broadcast the request to all the nodes in the second trial?}
%\wt{Then if a honest node didn't receive the 2nd trial, it wouldn't prevote in any case.}




% \subsubsection{List of Modifications to \sysname.}
% \label{sec:liveness-mod}

% \begin{enumerate}[label=\Alph*.,leftmargin=*]
%     \item Log Replication. 
%     \begin{enumerate}[label=\Alph{enumi}\arabic*.]
%         \item We enabled clients to raise a dispute against a faulty leader. This solves one of the liveness problems. 
%     \end{enumerate}
    
%     \item Leader Election. 
%     \begin{enumerate}[label=\Alph{enumi}\arabic*.]
%         \item We use prevote as a buffer of the voting process. This prevents Byzantine nodes from premissionlessly initiating new elections or skipping terms. 
        
%         \item We force synchronization of term numbers among honest nodes. In vanilla Raft, nodes may have various term numbers and a Byzantine node may override a successful election by picking a high term number. 
        
%         \item We assign one unique candidate to each term, and ensures that as the term number increments $n$ times, each node becomes candidacy exactly once. This guarantees that even in the worst case where there exists only 1 candidate eligible for leadership, the election can still end. 
%     \end{enumerate}
    
% \end{enumerate}

% \subsubsection{List of Prevote Conditions.}
% \label{sec:liveness-prevote}

% \begin{enumerate}[label=\Alph*.]
%     \item As a follower admitting a leader. 
%     \begin{enumerate}[label=\Alph{enumi}\arabic*.]
%         \item The leader fails to send a heartbeat before timeout \theart. 
        
%         \item The leader fails to respond within RPC before timeout \theart. 
        
%         \item The leader sends invalid data during RPC calls, such as unauthenticated requests, invalid certificates, and logs of invalid format. 
        
%         \item The leader fails to send a valid commitment certificate before timeout \treq since the request was forwarded by self. 
%     \end{enumerate}
    
%     \item As a follower during election. 
%     \begin{enumerate}[label=\Alph{enumi}\arabic*.]
%         \item The candidate fails to send a valid leader certificate before timeout \tvoter. 
        
%         \item The candidate sends invalid data, such as ill-formatted vote requests and leader certificates. 
%     \end{enumerate}
    
%     \item As a candidate: it receives $f+1$ vote rejections before timeout \tcand or fails to receive $f$ votes at timeout \tcand. 
%     % \begin{enumerate}[label=\Alph{enumi}\arabic*.]
%     %     \item The candidate receives $f+1$ vote rejections before timeout \tcand or fails to receive $f$ votes at timeout \tcand. 
%     % \end{enumerate}
% \end{enumerate}



\subsection{Theoretical Liveness Guarantee}

The following theorem shows that \sysnamelive achieves liveness. 
The proof is in Appendix \ref{sec:proof-availability}. 

\begin{theorem}
    We assume all clients will resubmit a request to the system within $\Delta$ time after one node admits a leader with a valid leader certificate.  
    After a client submits a request to \sysname at time $t = 0$, one of the two events will occur. 
    \begin{enumerate}
        \item The request will be committed at time $t = t'$ for some $t' < \infty$.
        \label{item:committed}
        
        \item The adversarial node can be accused by an auditor with irrefutable proof.
        \label{item:accused}
    \end{enumerate}   

    \label{thm:availability}
\end{theorem}

% \subsection{Discussions on \sysnamelive}

% Not surprisingly, fault tolerance does not come without expenses, but they are manageable for \sysnamelive. 
For practitioners, the decision to implement \sysnamelive or \sysname depends on the internal threat model. 
First of all, in client-leader disputes, an adversarial client may launch distributed denial-of-service (DDoS) attacks to spam follower nodes with dispute messages. 
However, DDoS threats are not specific to \sysnamelive; clients can already spam requests in vanilla Raft. 
% It is possible to alleviate this issue by designing access frequency limits that comprehensively deal with flooding requests and disputes, which is out of the scope of this paper. 
The prevote design also increases the communication complexity and affects performance during leader elections. 
However, leader elections do not occur often in practice and the size of broadcast prevote messages is constant. 
Finally, for round-robin election, the expected time complexity of an election is irrelevant (\sref{sec:proof-rr}) to $n$, 
which is asymptotically no worse than than in vanilla Raft. 
On the other hand, a Byzantine node can increase the time complexity of leader election up to linear in $n$, but vanilla Raft and \sysname are much worse---their elections cannot even proceed if the adversary keeps seizing leadership. 
The major weakness of \sysnamelive is its inability to generalize to multiple Byzantine nodes (more details in \S\ref{sec:discussion-live}). 
In the presence of two Byzantine nodes Alice and Bob, Alice can make sure Bob is the freshest  pass leadership to each other indefinitely. 
% We address that it is much difficult to tolerate multiple Byzantine nodes than to account for their faults, where the limitation for accountability is only related to the low cost of safety attacks. 
% If there are two Byzantine nodes in \sysnamelive, even if we raise the threshold count of prevotes from $2$ to $3$, they can indefinitely pass leadership to each other and effectively censor transactions. 
Understanding how to tolerate such faults is an interesting direction for future work.

% In summary, we still recommend system designers to implement \sysnamelive, but apply it only to small distributed systems (e.g., with 3 or 5 nodes). 
% In comparison to \sysname, it not only provides the same forensics support, but effectively prevents one single node from paralyzing the entire system, which significantly increases the costs of liveness attacks. 

% \gfa{Can we add some comments on how this will affect performance? A malicious client could use this to use up resources right (communication and computation)? Do we recommend organizations implement this? }

\subsection{Implementation Details}

We first outline the precise prevote conditions. Then we provide pseudocode for the new leader election process. 
\subsubsection{List of Prevote Conditions.} ~
\label{sec:liveness-prevote}

\begin{enumerate}
    \item As a follower admitting a leader. 
    \begin{enumerate}
        \item The leader fails to send a heartbeat before timeout \theart. 
        
        \item The leader fails to respond within RPC before timeout \theart. 
        
        \item The leader sends invalid data during RPC calls, such as unauthenticated requests, invalid certificates, and logs of invalid format. 
        
        \item The leader fails to send a valid commitment certificate before timeout \treq since the request was forwarded by self. 
    \end{enumerate}
    
    \item As a follower during election. 
    \begin{enumerate}
        \item The candidate fails to send a valid leader certificate before timeout \tvoter. 
        
        \item The candidate sends invalid data, such as ill-formatted vote requests and leader certificates. 
    \end{enumerate}
    
    \item As a candidate: it receives $f+1$ vote rejections before timeout \tcand or fails to receive $f$ votes at timeout \tcand. 
    % \begin{enumerate}[label=\Alph{enumi}\arabic*.]
    %     \item The candidate receives $f+1$ vote rejections before timeout \tcand or fails to receive $f$ votes at timeout \tcand. 
    % \end{enumerate}
\end{enumerate}


\subsubsection{Leader Election}

In Alg. \ref{alg:rf-elect}, we precisely define the protocol of the round-robin leader election in \sysnamelive (\sref{sec:liveness-design}). 

\begin{algorithm}[!htb]
\caption{Round-Robin Leader Election in \sysnamelive}
\label{alg:rf-elect}
\KwIn{Term $t$, node $v$}
\KwOut{New Term, New Leader}

% $M_v \leftarrow M$\;
\SetKw{Broadcast}{broadcast}

\Pn{\FVote{$t$, $v$}}{
    $\tau \leftarrow t$\;

    \While{\textbf{true}}{
        \textbf{Prevote:}\BlankLine
        \Broadcast $\sigma_{v}(\code{prevote}(\tau))$\;
        Wait indefinitely for $1$ {prevote} message %, or a multi-signed $\sigma_{U}(\code{prevote}(\tau))$ with $|U| \ge 2$\;
        \BlankLine
        \textbf{Vote:}\BlankLine
        $\tau \leftarrow \tau + 1$\;
        
        Start listener of $\sigma_{U}(\code{prevote}(\tau+1))$ with $|U| \ge 2$ (Jump to \textbf{PrevoteInterrupt})\;
        
        \If{$c_\tau = v$}{
            Start timed event (Jump to \textbf{Timeout} after \tcand)\;
            \Broadcast $\textsc{RequestVote}(v, (T, J))$\;
            Wait for signed votes $\sigma_{\cdot}(\textsc{RequestVote}(v, (T, J)))$ from $f+1$ nodes\;
            \Broadcast $\lcert = \sigma_{U}(\textsc{RequestVote}(v, (T, J)))$\;
            \KwRet{$\tau, v$}\;
        }\Else{
            Start timed event (Jump to \textbf{Timeout} after \tvoter)\;
            Wait for $\textsc{RequestVote}(c_{\tau}, (T, J))$\;
            \If{By $(T, J)$, $c_{\tau}$ is as fresh as $v$}{
                Vote for $c_\tau$ by sending $\textsc{RequestVote}(c_\tau, (T, J))$\;
            }\Else{
                Inform $c_\tau$ of rejection\;
            }
            Wait for multi-signed $\sigma_{U}(\textsc{RequestVote}(c_\tau, (T, J)))$\;
            \KwRet{$\tau, c_\tau$}\;
        }
        \BlankLine
        \textbf{Timeout:}\BlankLine
        \Continue\;\BlankLine
        \textbf{PrevoteInterrupt:}\BlankLine
        \Continue and skip \textbf{Prevote} of next iteration\;
    }
}

\end{algorithm}


\subsection{Limitations}
\label{sec:discussion-live}

By simply raising the threshold of prevotes, \sysnamelive still cannot tolerate Byzantine faults against liveness from more than one corrupt nodes. 
We present an attack launched by two nodes with labels $0$ and $f$, where $n = 2f+1$. 
Suppose node $0$ initially holds the leadership. 
It replicates some entries (without commitment) to only nodes from $f$ to $2f$, such that $f$ is the first node on the round-robin loop that is fresh enough to be elected. 
Then, it gives up leadership due to client complaints, allowing node $f$ to become the next leader. 
Node $f$ replicates some new entries to only nodes $0$ to $f$, making $0$  the first node that is fresh enough to be elected. 
After it falls from the client-leader dispute, the leadership passes to $0$ again. 
The entire process loops forever without a single log entry being committed. 

Note that it is impractical to exclude a fallen leader from future candidacy, because timeouts in the second trial occasionally happen to honest nodes in practice. 
Such design will greatly weaken the robustness of the entire system. 

